MVTrans: Multi-View Perception of Transparent Objects

Transparent object perception is a crucial skill for applications such as robot manipulation in household and laboratory settings. Existing methods utilize RGB-D or stereo inputs to handle a subset of perception tasks including depth and pose estimation. However, transparent object perception remains to be an open problem. In this paper, we forgo the unreliable depth map from RGB-D sensors and extend the stereo based method. Our proposed method, MVTrans, is an end-to-end multi-view architecture with multiple perception capabilities, including depth estimation, segmentation, and pose estimation. Additionally, we establish a novel procedural photo-realistic dataset generation pipeline and create a large-scale transparent object detection dataset, Syn-TODD, which is suitable for training networks with all three modalities, RGB-D, stereo and multi-view RGB. Project Site: https://ac-rad.github.io/MVTrans/

==> 0-preamble.tex <==
% Author: Animesh Garg
% Date : July 2015
% This is a list of common packages needed in a wide range of latex docs for everyday writing.
\usepackage{marginnote}
% ---------------------------------
%floats and figures
% ---------------------------------
\usepackage{graphics}
\usepackage{wrapfig}
\usepackage[pdftex]{graphicx}
\DeclareGraphicsExtensions{.pdf,.png,.jpg}
%\pdfimageresolution200

\usepackage[font=small,labelfont=bf]{caption}
\usepackage{subcaption}
%DONT USE BOTH SUBCAPTION AND SUBFIGURE
%\usepackage[center]{subfigure} 
% \usepackage{overpic}
\usepackage[rightcaption]{sidecap}
\usepackage{pbox}

% ---------------------------------
%Math Stuff
% ---------------------------------
\usepackage{mathtools}
% \usepackage{bbm}
\usepackage{amsmath, amssymb, amscd}
\usepackage{ wasysym } %special symbols
\usepackage{amsfonts}
\usepackage{mathptmx} % selects Times Roman as basic font
\usepackage{gensymb} 
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{mdwmath}
% \usepackage{mdwtab}
% \usepackage{eqparbox} %equations

% ---------------------------------
%Symbols
% ---------------------------------
\DeclareMathAlphabet{\mathcal}{OMS}{lmsy}{m}{n}
\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
\usepackage{textcomp} %for getting text tilde
%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\usepackage{dsfont}

% ---------------------------------
%  Algorithms
% ---------------------------------
% http://tex.stackexchange.com/questions/229355/algorithm-algorithmic-algorithmicx-algorithm2e-algpseudocode-confused

% \usepackage{algorithm} %float wrapper for algorithms. %dont use with algorithm2e
%should only use one of algorithmic or algorithmicx or algorithm2e
% \usepackage{algorithmic} %least preferred
% \usepackage[ruled,vlined,linesnumbered]{algorithm2e} 
% \usepackage{algorithmicx, algpseudocode} %algpseudocode:layout for algorithmicx

% ---------------------------------
%Table Stuff
% ---------------------------------
\usepackage{array} %for table entries to be in center of cell
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}

\usepackage[
  separate-uncertainty = true,
  multi-part-units = repeat
]{siunitx}
% ---------------------------------
%DOCUMENT WIDE
% ---------------------------------
\usepackage[T1]{fontenc} 
\usepackage[utf8]{inputenc}
\usepackage[english]{babel} %for hyphenation rules
\usepackage{units}
% \usepackage{siunitx}
\usepackage{bm}
\usepackage{times} % assumes new font selection scheme installed
\usepackage{outlines}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{xspace}
\usepackage{flushend}%balance columns on last page
% \usepackage[yyyymmdd,hhmmss]{datetime}
\usepackage{csquotes}
\usepackage{makeidx}
\usepackage{pdfpages}

\let\labelindent\relax
\usepackage{enumitem}

% \usepackage{fixltx2e} %fix latex issue across versions not needed in new latex versions
\usepackage{soul} %text highlighting
\usepackage{subfiles} %individual file compilation--makes it quick 

\usepackage[protrusion=true,expansion=true]{microtype}
\setlength{\emergencystretch}{3em}

\usepackage[yyyymmdd]{datetime}
\renewcommand{\dateseparator}{-}
\date{\protect\formatdate{1}{1}{2001}}

% ---------------------------------
%Bibliography and cross-ref
% ---------------------------------
% The following lines are for IEEE style conflicts with natbibs
% \makeatletter
% \let\NAT@parse\undefined
% \makeatother
% \usepackage[numbers]{natbib}
% \usepackage{cite} %DONT USE NATBIB AND CITE TOGETHER

%hyperlinking
\usepackage{url}
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother
\usepackage{color}
% \usepackage{xcdraw}
% \usepackage[usenames,dvipsnames,table]{xcolor}
\usepackage[table]{xcolor}
\usepackage[pagebackref=false,breaklinks=true,colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue,bookmarks=false]{hyperref}
\usepackage[capitalize, noabbrev]{cleveref}

%=======U S E R  D E F I N E D  M A C R O S=======
% \newcommand{\bibhref}[2]{#2}
\usepackage{soul} %text highlighting
\newcommand{\todohl}[1]{{[\hl{#1?}]}}

\newcommand{\todo}[1]{\textcolor{red}{[#1?]}}
\newcommand{\etal}{et al.~}
% \newcommand{\tocite}[1]{\textcolor{red}{[cite:#1?]}}
%takes in optional argument
\newcommand{\tocite}[1]{%
\textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
}

\newcommand{\ignore}[1]{}

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it

\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure\,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

% use this command instead of writing "da Vinci" so it's never split 
\newcommand{\argmin}{\operatornamewithlimits{arg\ min}}
\newcommand{\argmax}{\operatornamewithlimits{arg\ max}}
\newcommand{\numshapes}{17 }
\newcommand{\analyticname}{Analytic }

\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{property}{Property}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

%version in control in draft mode
% Simple and headings are two pagestyles in the ucbthesis class. May need edits to whatever different pagestyle is being used. 
\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}



% ---------------------------------
% USER defined macros: Space Tweaks
% ---------------------------------
\setlength{\abovecaptionskip}{2.5mm}
\setlength{\belowcaptionskip}{1.5mm} 
\setlength{\textfloatsep}{3mm}
\setlength{\dbltextfloatsep}{3mm}

%\renewcommand{\baselinestretch}{.9945} %space between lines - use as last resort
\renewcommand{\arraystretch}{1.15}

% Spacing before and after section headings
\usepackage{titlesec}
\titlespacing{\section}{0pt}{0.3\baselineskip}{0.25\baselineskip}
\titlespacing{\subsection}{0pt}{0.2\baselineskip}{0.15\baselineskip}
\titlespacing{\subsubsection}{0pt}{0.05\baselineskip}{0.03\baselineskip}

%% paragraph (fine tune spacing close to deadline)
\renewcommand{\paragraph}[1]{\vspace{1em}\noindent\textit{#1} --}
% \newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}



